SALSA: Attacking Lattice Cryptography with Transformers

Currently deployed public-key cryptosystems will be vulnerable to attacks by full-scale quantum computers. Consequently, "quantum resistant" cryptosystems are in high demand, and lattice-based cryptosystems, based on a hard problem known as Learning With Errors (LWE), have emerged as strong contenders for standardization. In this work, we train transformers to perform modular arithmetic and combine half-trained models with statistical cryptanalysis techniques to propose SALSA: a machine learning attack on LWE-based cryptographic schemes. SALSA can fully recover secrets for small-to-mid size LWE instances with sparse binary secrets, and may scale to attack real-world LWE-based cryptosystems.

==> header.tex <==
% Recommended, but optional, packages for figures and better typesetting:
\usepackage{microtype}
\usepackage{graphicx}
\usepackage{subfigure}
\usepackage{booktabs} % for professional tables
\usepackage{multirow}

% hyperref makes hyperlinks in the resulting PDF.
% If your build breaks (sometimes temporarily if a hyperlink spans a page)
% please comment out the following usepackage line and replace
\usepackage{hyperref}
\usepackage{caption}

% Attempt to make hyperref and algorithmic work together better:
\newcommand{\theHalgorithm}{\arabic{algorithm}}
\usepackage[multiple]{footmisc}

\RequirePackage{algorithm}
\RequirePackage{algorithmic}
\usepackage{amsmath,amsthm,amssymb,amscd,url,enumerate, mathtools}
\usepackage[utf8]{inputenc}
\usepackage{wrapfig}
\usepackage{pdflscape}
\usepackage{tikz}
\usetikzlibrary{decorations.markings,arrows}
\usepackage{tikz-cd}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{graphicx}
\usepackage{amsthm}
\usepackage{mathrsfs}
\usepackage{dsfont}
\usepackage{ulem}
\usepackage{enumitem}
\usepackage{array}
\usepackage{verbatim}
\newcolumntype{?}{!{\vrule width 1pt}}
\usepackage[capitalize,noabbrev]{cleveref}
\DeclareMathOperator*{\argmin}{arg\,min} 

\newcommand{\amod}{\!\! \pmod}
\newcommand{\legendre}[2]{\genfrac{(}{)}{}{}{#1}{#2}}

%%%%%%%% Set Up Theorem-Style Formats %%%%%%%%%%%%%% 
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}

\usepackage[textwidth=15mm, textsize=tiny]{todonotes}

\newcommand{\para}[1]{{\vspace{2pt} \bf \noindent #1}}  
\newenvironment{packed_itemize}{
\begin{list}{\labelitemi}{\leftmargin=1em}
\setlength{\itemsep}{1pt}                                                           
\setlength{\parskip}{0pt}                                                                                 \setlength{\parsep}{0pt}                                                                                  \setlength{\headsep}{0pt}                                                                                 \setlength{\topskip}{0pt}                                                                                 \setlength{\topmargin}{0pt}                                                                               \setlength{\topsep}{0pt}                                                                                  \setlength{\partopsep}{0pt}                                                                               }{\end{list}}                                                                                                                                  

\newenvironment{packed_enumerate}{  
\begin{enumerate}                                                                                         \setlength{\itemsep}{3pt}                                                                                 \setlength{\parskip}{0pt}                                                                                 \setlength{\parsep}{0pt}                                                                                  \setlength{\headsep}{0pt}                                                                                 \setlength{\topskip}{0pt}                                                                                 \setlength{\topmargin}{0pt}                                                                               \setlength{\topsep}{0pt}                                                                                  \setlength{\partopsep}{0pt}
}{\end{enumerate}} 
\newcommand{\Mod}[1]{\ (\mathrm{mod}\ #1)}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\FF}{\mathbb{F}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\Fp}{\mathbb{F}_p}
\newcommand{\Fpp}{\mathbb{F}_{p^2}}
\newcommand{\End}{\operatorname{End}}
\newcommand{\Disc}{\operatorname{Disc}}
\newcommand{\disc}{\operatorname{disc}}
\newcommand{\trd}{\operatorname{trd}}
\newcommand{\nrd}{\operatorname{nrd}}
\newcommand{\typ}{\operatorname{Typ}}
\newcommand{\Ells}{\operatorname{Ell}}
%\DeclareMathOperator{\End}{End}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\Cl}{Cl}
\DeclareMathOperator{\ells}{\mathcal{E}\ell\ell}
\DeclareMathOperator{\poly}{poly}
\DeclareMathOperator{\gal}{Gal}
\DeclareMathOperator{\pic}{Pic}
\DeclareMathOperator{\dist}{Dist}
\DeclareMathOperator{\lwe}{\textbf{LWE}}
\let\SS\relax   \DeclareMathOperator{\SS}{SS}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}

\definecolor{Bittersweet}{rgb}{1.0, 0.44, 0.37}
\definecolor{lightblue}{HTML}{4e7dd4}
\definecolor{lightgreen}{HTML}{117733}
\definecolor{lred}{HTML}{CC6677}
\definecolor{lyellow}{HTML}{DDCC77}

\newcommand{\MC}[1]{\textcolor{cyan}{{\sf } {\sl{#1}}}}
\newcommand{\EG}[1]{\textcolor{green}{{\sf (Evrard:} {\sl{#1})}}}
\newcommand{\FC}[1]{\textcolor{orange}{{\sf} {\sl{#1}}}}
\newcommand{\KL}[1]{\textolor{purple}{{\sf ({Kristin:} {\sl {#1})}}}}
\newcommand\EC[1]{{\color{lightgreen} Emily: \emph{#1}}}
\newcommand\emily[1]{{\color{lightgreen} #1}}
